Chaotic-to-Fine Clustering for Unlabeled Plant Disease Images

Current annotation for plant disease images depends on manual sorting and handcrafted features by agricultural experts, which is time-consuming and labour-intensive. In this paper, we propose a self-supervised clustering framework for grouping plant disease images based on the vulnerability of Kernel K-means. The main idea is to establish a cross iterative under-clustering algorithm based on Kernel K-means to produce the pseudo-labeled training set and a chaotic cluster to be further classified by a deep learning module. In order to verify the effectiveness of our proposed framework, we conduct extensive experiments on three different plant disease datatsets with five plants and 17 plant diseases. The experimental results show the high superiority of our method to do image-based plant disease classification over balanced and unbalanced datasets by comparing with five state-of-the-art existing works in terms of different metrics.

==> tables/data_distribution_cdd.tex <==
\begin{center}
\begin{scriptsize}
 \begin{tabular}{||p{0.15\textwidth}|p{0.07\textwidth}|p{0.07\textwidth}|p{0.07\textwidth}|p{0.07\textwidth}|p{0.07\textwidth}||} 
 \hline
 Cluster \# & 1 & 2 & 3 & 4 & 5 \\ [0.5ex] 
 \hline\hline
 K-means & 751 & 1128 & 1075 & 640 &  \\
 \hline
 KMM & 954 & 1398 & 786 & 548 &  \\
 \hline
 Spectral & 931 & 1075 & 894 & 580 &  \\
 \hline
 KIBICS & 697 & 1193 & 1383 & 314 &  \\
 \hline
 \end{tabular}
\end{scriptsize}
\end{center}

==> tables/data_distribution_pvps.tex <==
\begin{center}
\begin{scriptsize}
 \begin{tabular}{||p{0.15\textwidth}|p{0.1\textwidth}|p{0.1\textwidth}|p{0.1\textwidth}|p{0.1\textwidth}||} 
 \hline
 Cluster \# & 1 & 2 & 3 & 4 \\ [0.5ex] 
 \hline\hline
 K-means & 751 & 1128 & 1075 & 640 \\
 \hline
 KMM & 954 & 1398 & 786 & 548  \\
 \hline
 Spectral & 931 & 1075 & 894 & 580 \\
 \hline
 AROC & 631 & 2564 & 2260 & 279 \\
 \hline
 KIBICS & 697 & 1193 & 1383 & 314 \\
 \hline
 \end{tabular}
\end{scriptsize}
\end{center}

==> tables/mendeley_citrus_dataset.tex <==
\begin{center}
\footnotesize
 \begin{tabular}{||p{0.1\textwidth}|p{0.2\textwidth}|p{0.1\textwidth}||} 
 \hline
 Plant & Disease / Health & Image Amount \\ [0.5ex] 
 \hline\hline
 \multirow{5}{*}{Citrus} 
 & Black Spot & 172 \\ 
 & Canker & 164 \\
 & Greening & 205 \\
 & Healthy & 59 \\
 & Melanose & 14 \\
 \hline
\end{tabular}
\end{center}

==> tables/per_cluster_acc.tex <==
\begin{center}
\begin{scriptsize}
 \begin{tabular}{||p{0.12\textwidth}|p{0.08\textwidth}|p{0.08\textwidth}|p{0.08\textwidth}|p{0.08\textwidth}|p{0.08\textwidth}|p{0.08\textwidth}||} 
 \hline
 Algorithm & Clusters & Ave. & Max & Min & FPP & LPP \\
 \hline
 K-means & 30 & 0.981 & 1.000 & 0.812 & 0.367 & 0.033 \\
 \hline
 KKM & 30 & 0.982 & 1.000 & 0.804 & 0.433 & 0.033 \\
 \hline
 Spectral & 30 & 0.977 & 1.000 & 0.770 & 0.367 & 0.067\\
 \hline
 \multirow{6}{*}{AROC} 
 & 1 & 0.227 & 0.227 & 0.227 & 0.000 & 1.000 \\
 & 3 & 0.621 & 1.000 & 0.241 & 0.500 & 0.500 \\
 & 9 & 0.881 & 1.000 & 0.540 & 0.571 & 0.286\\
 & 11 & 0.923 & 1.000 & 0.540 & 0.600 & 0.200 \\
 & 11 & 0.945 & 1.000 & 0.540 & 0.714 & 0.143 \\
 & 13 & 0.964 & 1.000 & 0.540 & 0.706 & 0.118 \\
 \hline
 \multirow{4}{*}{FINCH} 
 & 1646 & 0.910 & 1.000 & 0.333 & 0.752 & 0.248 \\
 & 542 & 0.891 & 1.000 & 0.400 & 0.491 & 0.355 \\
 & 284 & 0.887 & 1.000 & 0.333 & 0.232 & 0.354\\
 & 283 & 0.853 & 1.000 & 0.333 & 0.138 & 0.450 \\
 \hline
 KIBICS-C & 30 & 0.958 & 1.000 & 0.587 & 0.300 & 0.100 \\
 \hline
 KIBICS-S & 30 & 0.959 & 1.000 & 0.587 & 0.267 & 0.100 \\
 \hline
 \end{tabular}
\end{scriptsize}
\end{center}

==> tables/per_cluster_acc_2.tex <==
\begin{center}
\begin{scriptsize}
 \begin{tabular}{||p{0.12\textwidth}|p{0.08\textwidth}|p{0.08\textwidth}|p{0.08\textwidth}|p{0.08\textwidth}|p{0.08\textwidth}|p{0.08\textwidth}||} 
 \hline
 Algorithm & Clusters & Ave. & Max & Min & FPP & LPP \\
 \hline
 K-means & 30 & 0.998 & 1.000 & 0.982 & 0.800 & 0.000 \\
 \hline
 KKM & 30 & 0.998 & 1.000 & 0.985 & 0.800 & 0.000 \\
 \hline
 Spectral & 30 & 0.998 & 1.000 & 0.983 & 0.767 & 0.000\\
 \hline
 \multirow{6}{*}{AROC} 
 & 1 & 0.315 & 0.315 & 0.315 & 0.000 & 1.000 \\
 & 3 & 0.719 & 0.993 & 0.440 & 0.000 & 0.667 \\
 & 9 & 0.998 & 1.000 & 0.990 & 0.556 & 0.000 \\
 & 11 & 0.998 & 1.000 & 0.990 & 0.636 & 0.000 \\
 & 11 & 0.998 & 1.000 & 0.990 & 0.636 & 0.000 \\
 & 13 & 0.998 & 1.000 & 0.990 & 0.692 & 0.000 \\
 \hline
 \multirow{4}{*}{FINCH} 
 & 1646 & 0.956 & 1.000 & 0.400 & 0.880 & 0.120 \\
 & 542 & 0.945 & 1.000 & 0.500 & 0.792 & 0.177 \\
 & 284 & 0.950 & 1.000 & 0.500 & 0.803 & 0.144\\
 & 283 & 0.951 & 1.000 & 0.500 & 0.802 & 0.141 \\
 \hline
 KIBICS-C & 30 & 0.985 & 1.000 & 0.550 & 0.967 & 0.033 \\
 \hline
 KIBICS-S & 30 & 0.869 & 1.000 & 0.348 & 0.333 & 0.400 \\
 \hline
 \end{tabular}
\end{scriptsize}
\end{center}

==> tables/plantvillage_dataset.tex <==
\begin{center}
\footnotesize
 \begin{tabular}{||p{0.1\textwidth}|p{0.2\textwidth}|p{0.1\textwidth}||} 
 \hline
 Plant & Disease / Health & Image Number \\ [0.5ex] 
 \hline\hline
 \multirow{4}{*}{Apple} & Scrab & 630 \\ 
 & Black Rot & 621 \\
 & Cedar Rust & 275 \\
 & Healthy & 1645  \\
 \hline
 Blueberry & Healthy & 1503  \\
 \hline
 \multirow{2}{*}{Cherry} & Healthy & 855 \\ 
 & Powdery Mildew & 1053 \\
 \hline
 
 \multirow{4}{*}{Corn} & Grey Leaf Spot & 514 \\
 & Common Rust & 1193 \\
 & Healthy & 1163 \\
 & Northern Leaf Blight & 986 \\
 \hline
 
 \multirow{4}{*}{Grape} & Black Rot & 1180 \\
 & Black Measles (Esca) & 1383 \\
 & Healthy & 423 \\
 & Leaf Blight & 1076 \\
 \hline
 
 Orange & Huanglongbing (Citrus Greening) & 5508  \\
 \hline
 \multirow{2}{*}{Peach} & Bacterial Spot & 2298 \\ 
 & Healthy & 361 \\
 \hline
 
 \multirow{2}{*}{Bell Pepper} & Bacterial Spot & 998 \\ 
 & Healthy & 1479 \\
 \hline
 
 \multirow{3}{*}{Potato} & Early Blight & 1001 \\ 
 & Healthy & 153 \\
 & Late Blight & 1001 \\
 \hline
 
 Raspberry & Healthy & 372  \\
 \hline
 
 Soybean & Healthy & 5091  \\
 \hline
 
 Squash & Powdery Mildew & 1836  \\
 \hline
 
 \multirow{2}{*}{Strawberry} & Healthy & 457 \\ 
 & Leaf Scorch & 1110 \\
 \hline
 
 \multirow{10}{*}{Tomato} & Bacterial Spot & 2128 \\ 
 & Early Blight & 1001 \\
 & Late Blight & 1910 \\
 & Leaf Mold & 953 \\
 & Septoria Leaf Spot & 1772 \\
 &  Two Spotted Spider Mite & 1677 \\
 &  Target Spot & 1405 \\
 &  Mosaic Virus & 374 \\
 &  Yellow Leaf Curl Virus & 5358 \\
 &  Healthy  & 1592 \\
 \hline
\end{tabular}
\end{center}

==> tables/precision_table_2.tex <==
\begin{center}
\begin{scriptsize}
 \begin{tabular}{||p{0.12\textwidth}|p{0.06\textwidth}|p{0.08\textwidth}|p{0.06\textwidth}|p{0.06\textwidth}|p{0.06\textwidth}|p{0.06\textwidth}|p{0.06\textwidth}||} 
 \hline
 Algorithm & Thresh & Clusters & PRE & Rec & F1 & NMI & PUR \\ [0.5ex] 
 \hline\hline
 K-means & N/A & 30 & 0.995 & 0.162 & 0.278 & 0.222 & 0.413  \\
 \hline
 KKM & N/A & 30 & 0.995 & 0.165 & 0.283 & 0.200 & 0.431  \\ 
 \hline
 Spectral & N/A & 30 & 0.995 & 0.159 & 0.274 & 0.205 & 0.428   \\
 \hline
 \multirow{6}{*}{AROC}
  & 10 & 1 & 0.216 & \textbf{1.000} & 0.355 & 0.003 & 0.315 \\
  & 1.5 & 3 & 0.474 & \textbf{1.000} & 0.644 & 0.383 & 0.493 \\
  & 0.4 & 9 & \textbf{0.996} & 0.995 & 0.996 & \textbf{0.898} & \textbf{0.915} \\
  & 0.2 & 11 & \textbf{0.996} & 0.995 & 0.995 & 0.896 & \textbf{0.915} \\
  & 0.1 & 11 & \textbf{0.996} & 0.995 & 0.995 & 0.896 & \textbf{0.915} \\
  & 0.05 & 13 & \textbf{0.996} & 0.992 & 0.994 & 0.896 & \textbf{0.915} \\
 \hline
 \multirow{4}{*}{FINCH} 
  & N/A & 1646 & 0.919 & 0.002 & 0.004 & 0.005 & 0.315 \\
  & N/A & 542 & 0.924 & 0.009 & 0.017 & 0.023 & 0.321 \\
  & N/A & 284 & 0.917 & 0.025 & 0.049 & 0.053 & 0.335 \\
  & N/A & 283 & 0.917 & 0.025 & 0.049 & 0.051 & 0.334 \\
 \hline
 KIBICS-C & N/A & 30 & 0.980 & 0.002 & 0.004 & 0.890 & 0.101 \\
 \hline
 KIBICS-S & N/A & 30 & 0.469 & 0.177 & 0.257 & 0.137 & 0.374 \\
 \hline
\end{tabular}
\end{scriptsize}
\end{center}

==> tables/pvps_details.tex <==
\begin{center}
\footnotesize
 \begin{tabular}{||p{0.1\textwidth}|p{0.2\textwidth}|p{0.1\textwidth}||} 
 \hline
 Plant & Disease / Health & Image Amount \\ [0.5ex] 
 \hline\hline
 \multirow{2}{*}{Peach} & Bacterial Spot & 2298 \\ 
 & Healthy & 361 \\
 \hline
 \multirow{2}{*}{Strawberry} & Healthy & 457 \\ 
 & Leaf Scorch & 1110 \\
 \hline
\end{tabular}
\end{center}

==> tables/rdd_precision_table.tex <==
\begin{center}
\begin{scriptsize}
 \begin{tabular}{||p{0.12\textwidth}|p{0.06\textwidth}|p{0.08\textwidth}|p{0.06\textwidth}|p{0.06\textwidth}|p{0.06\textwidth}|p{0.06\textwidth}|p{0.06\textwidth}||} 
 \hline
 Algorithm & Thresh & Clusters & PRE & Rec & F1 & NMI & PUR \\ [0.5ex] 
 \hline\hline
 K-means & N/A & 5 & 0.558 & 0.353 & 0.433 & 0.238 & 0.542  \\
 \hline
 KKM & N/A & 5 & 0.625 &0.391 & 0.481 & 0.229 & 0.508 \\ 
 \hline
 Spectral & N/A & 5 & 0.597 & 0.359 & 0.448 & 0.327 & 0.700  \\
 \hline
 \multirow{3}{*}{AROC}
  & 100 & 1 & 0.328 & \textbf{1.000} & \textbf{0.494} & 0.015 & 0.392 \\
  & 1 & 1 & 0.328 & \textbf{1.000} & \textbf{0.494} & 0.015 & 0.392 \\
  & 0.001 & 1 & 0.328 & \textbf{1.000} & \textbf{0.494} & 0.015 & 0.392 \\
 \hline
 \multirow{3}{*}{FINCH} 
  & N/A & 41 & 0.743 & 0.044 & 0.084 & 0.035 & 0.425 \\
  & N/A & 17 & 0.767 & 0.174 & 0.283 & 0.198 & \textbf{0.592} \\
  & N/A & 15 & 0.741 & 0.191 & 0.304 & 0.189 & 0.575 \\
 \hline
 KIBICS-C & N/A & 8 & 0.719 & 0.247 & 0.367 & 0.202 & 0.508 \\
 \hline
 KIBICS-S & N/A & 5 & \textbf{0.773} & 0.225 & 0.367 & \textbf{0.325} & 0.458 \\
 \hline
 KIBICS & N/A & 5 & 0.657 & 0.254 & 0.366 & 0.212 & 0.483 \\
 \hline
\end{tabular}
\end{scriptsize}
\end{center}

==> tables/traditional_clustering_algorithms.tex <==
\begin{center}
\footnotesize
 \begin{tabular}{||p{0.15\textwidth}|p{0.15\textwidth}||} 
 \hline
 Algorithm name & Catagory \\ [0.5ex] 
 \hline\hline
 K-means & Partitional \\ 
 \hline
 CLARA & Partitional  \\
 \hline
 Hierarchical & Linkage \\
 \hline
 EM & Model-based  \\
 \hline
 HC-Model & Model-based  \\
 \hline
 Spectral & Spectral methods \\ 
 \hline
 Subspace & Subspace-based \\
 \hline
 OPTICS & Density \\
 \hline
 DBSCAN & Density \\
 \hline
\end{tabular}
\end{center}

==> tables/uci_rice_disease_dataset.tex <==
\begin{center}
\footnotesize
 \begin{tabular}{||p{0.2\textwidth}|p{0.4\textwidth}|p{0.2\textwidth}||} 
 \hline
 Plant & Disease / Health & Image Number \\ [0.5ex] 
 \hline\hline
 \multirow{3}{*}{Rice} 
 & Bacterial Leaf Blight & 41 \\ 
 & Brown Spot & 41 \\
 & Leaf Smut & 41 \\
 \hline
\end{tabular}
\end{center}
